Efficient Routing for Quantum Key Distribution Networks

As quantum key distribution becomes increasingly practical, questions of how to effectively employ it in large-scale networks and over large distances becomes increasingly important. To that end, in this work, we model the performance of the E91 entanglement based QKD protocol when operating in a network consisting of both quantum repeaters and trusted nodes. We propose a number of routing protocols for this network and compare their performance under different usage scenarios. Through our modeling, we investigate optimal placement and number of trusted nodes versus repeaters depending on device performance (e.g., quality of the repeater's measurement devices). Along the way we discover interesting lessons determining what are the important physical aspects to improve for upcoming quantum networks in order to improve secure communication rates.

==> old-sim.tex <==
\subsection{Simulator}
\begin{figure}
    \centering
    \includegraphics{sideguide.pdf}
    \caption{A legend for Figure \#\ref{fig:stages1-3}. (a) denotes a node in the network, specifically a repeater with 4 (b) connection terminals from which entangled photons are sent and received over (c) fiber optic connections between other repeaters and (d) trusted nodes. Below the line, an entangled channel (e) connecting multiple trusted nodes through intra-node entanglement (f)}
    \label{fig:guide}
\end{figure}

%%wb, 4/20/20, put three figures in stages 1-3 side by side 
\triplefig{stage1.pdf}{Stage 0}{stage2.pdf}{Stage 1}{stage3.pdf}{Stage 2}{(a) The initial network, in a 5x5 grid, with a central trusted node (T) between Alice (A) and Bob (B), as discussed in stage 0. (b) A possible network configuration after stage 1, in which some nodes succeed in establishing a shared EPR pair with their neighbors over the fiber channels and some do not. Note that there are a number of possible paths between A, B and T. (c) Successful entanglement chaining and routing (depicted as the intra-repeater connections) as discussed in stage 2. In this graph, routing has resulted in a channel being created between each pair of A, B and T. These routes are successful and coherent only if every bell state measurement along the path succeeds, and if no decohering occurs in the path, so minimizing the path lengths with effective routing algorithms and trusted node utilization is advantageous. For the purposes of this diagram we condition on the channels remaining coherent, but in practice any could have become decoherent.}{stages1-3}
To analyze the behavior of the QKD network we envision and to evaluate the performance of the various routing protocols we construct later, we wrote a custom simulator.  This simulator, following an initialization stage, operates in four steps, which each  take in as input the state of the network graph at the end of the state prior and outputting the resulting, evolved graph. \par
\textbf{0. Initialization:}
Consider an $N\times N$ (for an odd $N$) network graph with some number of trusted nodes and Alice and Bob at opposite corners of the network, Such a network begins in the state $G = \{V,E\}$ where $V = \{0,1, \dotso,N^2-2, N^2-1\}$ with Alice at node $A=0$ and Bob at node $B = N^2-1$, and trusted nodes $T \subseteq V$. Finally, without loss of generality we consider a grid network in which the nodes are ordered increasing from left to right and bottom to top, and so we have $E$ defined in the natural way. We show the steps describing the evolution of this graph in the following section, as well as the evolution of this example graph in Figs.~\ref{fig:stages1-3} and \ref{fig:stage5}, with a key provided in Fig.~\ref{fig:guide}. \par
\textbf{1. Entanglement Generation:} In the initial phase, each node attempts to share one half of a  Einstein–Podolsky–Rosen (EPR) \cite{EPR} pair with its neighbors over the fiber channel. The photon pair is successfully transmitted and received with probability $10^{-\alpha L/10}$ \cite{transmittance} where $\alpha$, also a characteristic of the network, is the transmittance of the fiber channel. As such the network evolves to $G_1 = \{V, E_1\}$ where $E_1 = \{(u,v) \forall (u,v) \in E  \; |\;  S(u,v) \}$  \OA{what is set notation for random sets?}, where $S(u,v)$ is a random binary function that returns true for any edge with probability $10^{-\alpha L/10}.$ \par
\textbf{2. Routing and Entanglement Chaining: } With the evolved network graph, the repeater nodes utilize a routing algorithm (we will discuss a number of candidate algorithms in the following section) to determine, at each repeater, which neighbors should be connected by entanglement. The routing algorithm, $R1$, takes $G_1$ as input and outputs $P = \{p_i\}_{i=0}^n$ where $p_i = (r_0^i, r_1^i, \dotso, r_{m_i}^i)$ describe paths originating from and ending at Alice, Bob, or a trusted node through a path of $m-2$ entanglement connected quantum repeaters. The quantum repeaters then use this pathing information and conduct bell state measurements on the photons they hold that are entangled with photons at the nodes before and after them in a path \bing{this sentence is a bit long; can we rephrase by using the notation?}, succeeding with probability $B$ and becoming decoherent with probability $D$. As a result of this action, the network evolves and is compromised of Alice, Bob, trusted nodes, and shared entanglement (which with some probability has decohered) between those parties. Specifically, we have $G_2 = \{V_2, E_2\}$ where $V_2 = T\cup \{A,B\}$ and $E_2 = \{(r_0^i,r_{m_i}^i,F(p_i)) \; \forall p_i \in P\}$ where $F(p_i)$ is a random binary function that decides whether or not the entangled channel has fidelity. Fidelity is maintained with probability $(1-d)^{m_i-2}$, as it must be the case that at each of the $m_i-2$ intermediate nodes, the bell state measurement did not fail. We note that as there can be multiple (up to two) paths between the same pair of entities, the elements in $E_2$ are not necessarily unique. \par
\textbf{3. Quantum Key Distribution:} In this stage, the entities in $G_2$ attempt to use the quantum channels established between them to conduct a round of an entanglement based QKD protocol --- in our case, E91. Here we will  introduce a secondary network structure, with weighted edges connecting Alice, Bob, and trusted nodes with weights representing the amount of key material shared between nodes. The edges additionally have associated with them a bit string, with length equal to their weight, representing whether there is a correlation in each bit of key material (though the value of the bits themselves, for the purpose of our simulation, is irrelevant). This graph, at the start of the protocol, is initialized to $G_3 = \{V_2, E_3\}$ where $E_3 = \{(u,v,0,\epsilon) \; \forall u,v \in V_2\},$ where $\epsilon$ is the empty string denoting the correlations in the amount of stored key material, which is 0 \bing{what does the `0' represent here?}.   

On this stage, we build on $G_3$ based on the state of $G_2$. Specifically, if QKD succeeds between two linked nodes, which it does with probability $\frac{1}{4},$ then a bit is added to that that bank of key material, which is a correlated with full probability if the link was coherent \bing{rephrase?}. If the link was not coherent, then we assume that it became a fully mixed state, and that resulting measurements are random and therefore correlated with $\frac{1}{2}$ probability. Formally, this means that for each edge $(u,v,1) \in E_2$, with $\frac{1}{4}$ probability we update the corresponding edge $(u,v,k,c)$ in $E_3$ to $(u,v,k+1,c||0)$, and likewise for each edge $(u,v,0)$ we update the corresponding edge to $(u,v,k,c||0)$ or $(u,v,k,c||1)$  with equal probability, where $||$ denotes concatenation of bit strings.

\par
\textbf{4. Key Distillation}
Stages 1-3 repeat some $M$ times, building sufficiently sized key stores between each of the participating parties in our network until, on this stage, the final key-distillation and key-routing process occurs. On this stage, each pair of parties that share some amount of raw key material can conduct standard post-processing procedures, namely, error correction and privacy amplification, to transform their raw-key stores into secret-key stores. As we are limiting our analysis in this work to only consider the performance in the asymptotic key-length realm, we do not consider finite key effects, and so the simulator simply transforms the edges $(u,v,k,c)$ in $G_3$ to be $(u,v,(1-2h(Q))k, \epsilon)$, to signify the error correction and privacy amplification process according to the standard process, where Q is the quantum bit error rate of the key, calculated as $\frac{w(c)}{k}$, where $w(x)$ signifies the Hamming weight of the bit string $x$ and where $h(x)=x\log(x)-(1-x)\log(1-x)$ is the binary entropy function. 
Following this process, the network conducts the final routing process on $G_4$, obtained through the above transformations of edges, in an effort to route the maximum amount of key material from Alice to Bob. To do this, we use a standard max-flow algorithm, in which any flow of $n$ key-bits from node $a$ to node $b$ going through node $c$ signifies node $c$ publishing the XOR of $n$ bits from its key stores shared with $a$ and $b$ respectively, and then discarding those $n$ bits. Nodes $a$ and $b$ can then of course recover this key material, pushing it through the network until we culminate with the maximal amount of key material being shared by Alice and Bob. 


% \iffalse 
% \begin{figure}
%     \centering
%     \includegraphics{stage1.pdf}
%     \caption{The initial network, in a 5x5 grid, with a central trusted node (T) between Alice (A) and Bob (B), as discussed in stage 0.}
%     \label{fig:stage1}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics{stage2.pdf}
%     \caption{A possible network configuration after stage 1, in which some nodes succeed in establishing a shared EPR pair with their neighbors over the fiber channels and some do not. Note that there are a number of possible paths between A, B and T.  }
%     \label{fig:stage2}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics{stage3.pdf}
%     \caption{Successful entanglement chaining and routing (depicted as the intra-repeater connections) as discussed in stage 2. In this graph, routing has resulted in a channel being created between each pair of A, B and T. These routes are successful and coherent only if every bell state measurement along the path succeeds, and if no decohering occurs in the path, so minimizing the path lengths with effective routing algorithms and trusted node utilization is advantageous. For the purposes of this diagram we condition on the channels remaining coherent, but in practice any could have become decoherent. }
%     \label{fig:stage3}
% \end{figure}
% \fi 

\begin{figure}
    \centering
    \includegraphics{stage5.pdf}
    \caption{$G_3$ being modified, as discussed in stage 3, where $k_i$ denotes the number of key bits already shared between two nodes, and $c_i$ denotes the correlation bit string. This diagram assumes that QKD was successful on each of the error free channels established in Figure \ref{fig:stages1-3}(c).}
    \label{fig:stage5}
\end{figure}
% Stages 1-3 repeat some $M$ times, building sufficient key stores between each the participating parties in our network until, on this stage, the final routing and distillation of key material occurs. \OA{assuming we just go with simple trusted nodes here, and leave regular to journal if not in this one} On this stage, the network conducts a standard max-flow algorithm, with a slight variation, to determine how to route the maximum amount of key material from Alice to Bob through the weighted edges present in the graph. To "push" $n$ bits key material from Alice, through a trusted node, to Bob, the trusted node must first share at least $n$ bits of key material with both Alice and Bob. The trusted node then XORs the $n$ bit  key strings and publishes them, so that Alice and Bob can recover each others raw-key strings. Here it becomes clear why it is necessary that these intermediary nodes be trusted, as they, unlike the repeaters, are the only parties other than Alice and Bob that have full information on the key strings. Additionally, it is worthwhile to note that this XORing process can result in cascading errors when routing raw key material, and so we cannot simply chain trusted nodes infinitely using this method. For completeless, we look at how the secondary network graph evolves during this stage. Consider any two flows pushing $n$ bits from node $u$ through node $v$ to node $w$, the corresponding edges in $G_4$, which are originally equal to the edges of $G_3$, are updated from $(u,v,k_1, c_1),(v,w,k_2, c_2)$, and $(u,w,k_3, c_3)$ to
% $(u,v,k_1-n,c_1||_0^{k_1-n}),(v,w,k_2-n,c_2||_0^{k_2-n})$, and
% $(u,w,k_3+n, c_3 || (c_1 ||_{k_1-n}^{k_1} \oplus c_2 ||_{k_2-n}^{k_2})).$ 
% To allow this error information to cascade through the whole network we change the max-flow algorithm slightly so that, rather than executing each flow, we execute one flow, update the graph, and then re-run the algorithm. We repeat this until no more key-material can be pushed from Alice to Bob, and then we proceed with standard post-processing procedure: namely, error-correction and privacy amplification. 

% As in this work we only analyze the performance of this network in the asymptotic case, we do not concern ourselves with any finite key effects, and can instead calculate the overall key rate, as is standard,to be $1-2h(Q)$ where $h(x) = xlog(x) - (1-x)log(1-x)$ is the binary entropy function and $Q = \frac{w(c)}{K}$ where $w(x)$ is the hamming weight function and $c$ and $K$ are the bit string and weight associated with the edge connecting Alice and Bob in the finalized $G_4$ graph.


==> routing-old.tex <==
During the second stage of the network evolution, we attempt to link parties in our network through a chain entanglement links at quantum repeaters between the parties. To determine which neighbors a repeater should connect, we utilize a routing algorithm, and we compare the performance of three variations of the algorithm to better understand the performance of the network when operating under different assumptions.

We consider two forms of routing algorithms in this work: global and local.  For algorithms with global information, we assume the system performing the routing decisions has full information on the state of the network in the second stage of its evolution; namely, the routing algorithm is given $G_1$, the network graph where edges imply the two connected nodes share a state of the form in Equation \ref{eq:shared-state}.  For the local case, each repeater has only local information on its own internal state (namely, it knows which of its neighbors it has shared a quantum state with, but it knows nothing beyond this) and must make decisions for itself based only on this information.  Clearly global routing algorithms will have greater opportunity to choose optimal paths for the entire network, however each node in the network must broadcast its state before a decision can be made.  Local routing algorithms, though potentially making sub-optimal decisions, may make these decisions immediately without waiting for state information from the entire network.  We propose in this section one global algorithm and two local algorithms.
\iffalse
\doublefigbig{NIA_annotated.pdf}{Local: NIA}{IA_annotated.pdf}{Local: IA}{(a) Shows a possible route that the Non-intersection Avoidant algorithm may choose, with two highlighted areas in which there were two equal paths, along with the distances between each neighbor and each trusted node that will be used to make routing decisions (b) Shows the same, for the Intersection Avoidant path. We note that in (b), as opposed to (a), at location (i), the IA algorithm will always make the correct decision, choosing to keep the path straight, and as such not cutting off the second path to T or ending the path up to location (ii).  In (a), this is a random choice. Conversely, while the global algorithm (not shown) would always connect the bottom and left neighbors at (ii), creating a path from A to B, to the Local algorithms, all three possible connections are equal regardless of the fact that the choices shown here result in no path being formed. \bing{I have troubling understand this example. Can you add the global routing algorithm for this example? It would be good to describe the example in the text in detail as well. You can refer to this example when illustrating the global algorithm. Similarly, refer to it when illustrating the other two algorithms. Then say explicitly how one is better than the other.}}{Routing}
\fi


\triplefigbig{NIA_annotated.pdf}{Local: NIA}{IA_annotated.pdf}{Local: IA}{Global.pdf}{Global}{(a) Shows a possible route that the Non-intersection Avoidant algorithm may choose, with two highlighted areas in which there were two equal paths, along with the distances between each neighbor and each trusted node that will be used to make routing decisions (b) Shows the same, for the Intersection Avoidant path. And (c), the result of using the global algorithm to find the shortest paths between trusted nodes. We note that in (b), as opposed to (a), at location (i), the IA algorithm will always make the correct decision, choosing to keep the path straight, and as such not cutting off the second path to T or ending the path up to location (ii).  In (a), this is a random choice. Conversely, in (c) the global algorithm chooses to connect the bottom and left neighbors at (ii), creating a path from A to B. To the Local algorithms, however,  all three possible connections are equal regardless of the fact that the choices shown here result in no path being formed. }{Routing}

\subsection{Routing with Global Information}

The first routing algorithm makes use of global link level information, such that on each iteration the repeaters know which connections in the network have succeeded and which have failed. Towards this end, inspired by (CITE) for entanglement distribution, we propose a greedy algorithm which attempts to ensure that the shortest possible paths between trusted nodes are utilized, maximizing the probability that successful connections are established, and minimizing the expected error rate of those connections. To do this it simply outputs the shortest path between any two parties (choosing randomly between paths of equal length), removes those edges from the graph, and repeats until there are no new paths remaining. We will note here this in this work we do not make any claims to the optimality of this or the later routing algorithms we will discuss, we simply analyze their performance. \iffalse The psuedocode for this algorithm is provided in \ref{alg:global}.

\begin{algorithm}[H]
    \caption{Global Algorithm:}
	\begin{algorithmic}[1]
	\State Let $G$ be the network state, $T$ be the set of trusted nodes, and $A$,$B$ be the nodes at which Alice and Bob are located.
	\State Let $sp_G(u,v)$ be a routine that returns the shortest path in $G$ between nodes $u$ and $v$.
	\State Let $P = \{(t_1,t_2)\; \forall t_1,t_2 \in (T\cup \{A,B\})\;  | \; t_1>t_2\}$
	\State Let $x \overset{\$}{\leftarrow} A$ denote selecting an element $x$ from set $A$ with uniform probability. 
	\While{True}
	    \State Let $S = \{sp_G(t_1,t_2) \; \forall (t_1,t_2) \in P\}$
	    \If{$S == \emptyset$}
	        \State Break.
	    \EndIf
	    \State Let $m_s = \underset{s \in S}{min} \; length(s)$.
	    \State Let $M = \{s \; \forall s \in S \; |  \;  length(s) == m_s\}$.
	    \State Let $p \overset{\$}{\leftarrow} M$.
	    \State Remove edges in $p$ from $G$.
	    \State Output path $p$ as a path to be attempted.
	 \EndWhile
    \end{algorithmic}
    \label{alg:global}
\end{algorithm}
\fi

Allowing the network to route with global network information is beneficial, but it is also impractical. Without perfect quantum memories, it is infeasible to store the entangled qubits at each repeater for a sufficiently long period of time to propagate network information to each repeater in the network --- even with perfect memories, the propagation would increase the complexity and latency of the network. The global algorithm still serves as a useful benchmark to compare with other algorithms that only utilize local link information.

\subsection{Routing with Local Information}

%  \begin{algorithm}
%     \caption{Local Algorithm (NIA/IA):}
% 	\begin{algorithmic}[1]
% 	    \State Let $d_{ij}$ denote the distance in hops between nodes $i$ and $j$ in the original network graph.
% 	    \State Let $neighbors(u)$ denote the set of neighbors of $u$ that share with $u$ an EPR pair.
% 	    \State Let $x \overset{\$}{\leftarrow} A$ denote selecting an element $x$ from set $A$ with uniform probability. 
% 	    \ForEach{repeater node $w$}
% 	        \If{$neighbors(w) \leq 1$}
% 	            \State Continue.
% 	        \EndIf
% 	        \State Let $nT_1 = \{(u,t) \forall u\in neighbors(w), \forall t \in T\cup{A,B} \}$
% 	        \State Let $d_1 = \underset{(u,t) \in nT_1}{min}d_{ut}$
% 	        \State Let $(v_1,t_1) \overset{\$}{\leftarrow} \{(u,t) \in nT_1 \; | \; d_{ut} == d_1\}$
	        
% 	        \State Let $nT_2 = \{(u,t) \in nT_1 \; | \; t \neq t_1\}$
% 	        \State Let $d_2 = \underset{(u,t) \in nT_2}{min}d_{ut}$
% 	        \State Let $P = \{(u,t) \in nT_2 \; | \; d_{ut} == d_2\}$
%     	    \If{IA}
%     	        \State If possible, filter $P$ to only contain pairs where the neighboring node is "in-line" with neighbor $v_1$, if not, do not filter.
%     	    \EndIf
%     	    \State Let $(v_2,t_2) \overset{\$}{\leftarrow} P$
%     	    \If{$v_1 == v_2$}
%     	        \State Let $nT_3 = \{(u,t) \in nT_1 \; | \; u \neq v_1 \wedge  t \neq t_2\}$
%     	        \State Let $nT_4 = \{(u,t) \in nT_2 \; | \; u \neq v_1 \wedge  t \neq t_1\}$
    	        
%     	        \State Let $d_3 = \underset{(u,t) \in nT_1}{min}d_{ut}$
%     	        \State Let $(v_3,t_3) \overset{\$}{\leftarrow} \{(u,t) \in nT_3 \; | \; d_{ut} == d_3\}$
    	        
%     	        \State Let $d_4 = \underset{(u,t) \in nT_4}{min}d_{ut}$
%     	        \State Let $(v_4,t_4) \overset{\$}{\leftarrow} \{(u,t) \in nT_4 \; | \; d_{ut} == d_4\}$
    	        
%     	       \State Replace either $(v_1,t_1,d_1)$ or $(v_2,t_2,d_2)$ with $(v_3,t_3,d_3)$ or $(v_4,t_4,d_4)$ respectively to minimize the sum $d_1+d_2$. If the cases are equal, choose to replace either one with equal probability. 
%     	   \EndIf
%       	   \State Conduct a Bell state measurement at node $w$ to connect neighbors $v_1$ and $v_2$
%     	   \State Remove nodes $v_1$ and $v_2$ from $neighbors(w)$
%     	   \If{$|neighbors(w)| == 2$}
%     	        \State Conduct a Bell state measurement at node $w$ to the remaining two neighbors of $w$
%     	   \EndIf
    	    
    	    
% 	    \EndFor
%     \end{algorithmic}
%     \label{alg:local}
% \end{algorithm}
% We analyze two such algorithms, closely related, in this work. The first algorithm, adapted from the local routing algorithm proposed in \cite{entanglement-nature}, has each repeater attempt to connect its neighbors that, in the original network configuration, have the shortest distance to two unique parties. Where there are choices that are equal in this sense, the first algorithm will choose between them at random. The second algorithm operates much the same as the first one, save for this random choice. Before choosing at random, the second algorithm attempts to limit the likelihood of intersecting another possible path in the graph by filtering out its final options to limit the number of right angles in the path. For this reason, we will refer to the second algorithm as being Intersection-Avoidant (IA), and the first one as being Non-Intersection-Avoidant (NIA). Specifically, these algorithms operate as shown in Algorithm \ref{alg:local}. \OA{might be better to have the algs in an appendix?} \WK{no, I prefer to avoid appendices in papers, but I think you can describe the intuition more maybe or how they operate in words before referring to the pseudo-code}

We analyze two such algorithms, closely related, in this work. The first algorithm is adapted from the local routing algorithm proposed in \cite{pant2019routing}, in which they solve a similar routing problem which for networks that do not include a concept of trusted nodes. Our extension of their algorithm, then, operates as follows: 

Each repeater knows the number of hops each neighbor is from Alice, Bob, or a trusted node in the network (though, unlike the global algorithm, they do not know if all those links share an entanglement of course). On a given iteration, each repeater (only repeaters take action in this stage) will check how many of its four immediate neighbors it shares a quantum state with (of the form in Equation \ref{eq:shared-state}. If it connected with fewer than two: it does nothing (as it is only a ``dead-end''); if it connected with two neighboring nodes, it simply connects the two. If a repeater has established a quantum state with more than two of its neighbors, it connects the two neighbors that have the shortest distance (in terms of hops in the network) to two unique end-users (by which we mean Alice, Bob, or trusted nodes, and which have a distance of 0 from themselves). This is in an effort to ensure that the path consisting of two end-users is the shortest possible path between them, without the advantage of having global information. In the case when two potential sets of connections are equal in distance, the algorithm chooses randomly between them in the interests of symmetry.  Following this, if there remain two neighbors that have not been utilized (i.e., this node established a quantum state with all four of its neighbors initially), the repeater connects the remaining two neighbors. We call this the \emph{Non-Intersection Avoidant (NIA)} algorithm (the choice of name will become clear momentarily). 

Our second proposed local routing algorithm operates similar to the first NIA, but with a single modification to one of the rules which, we will come to see later, has a tremendous effect on performance.  In the case that a repeater must choose between two sets of potential connections (that is, the repeater has established a quantum state with three or four of its neighbors), we bias towards connections that do not create a right-angle in the network graph, in favor of connections between nodes that are "in line" with each other. This has the effect of simplifying the paths that are created in our graph, and limiting the number of times one path utilizes an edge that was integral to the formation of another path, but not to the formation of itself. We call this second local algorithm "Intersection Avoidant" (IA). %We provide psuedocode for both algorithms in Algorithm \ref{alg:local}.

In Fig. ~\ref{fig:Routing}, we show the resulting routes as chosen be each of the three algorithms, operating on the same set of EPR pairs. In Fig. ~\ref{fig:Routing}(a), the NIA algorithm makes two non-optimal decisions, at locations (i) ad (ii). At location (i), the repeater attempts to connect node A (as that node has a minimum distance of 0 from a party node, itself) with one of the other two neighbors of node (i). Each of the neighbors are equally close to the closest unique party node, and so the NIA selects one at random. In our example, the algorithm chooses to connect the neighbor to the right. While the algorithm still manages to connect A and T, this decision has two negative impacts. First, it renders a possible path between A and T beginning to the right of A useless, wasting those EPR pairs. At the same time, it also cuts off the any paths between A and B or T that go through nodes above (i). In (b), we see that this is remedied. Because the IA algorithm chooses "straight" paths when faced with two otherwise equal paths, node (i) makes the correct decision to path upwards, allowing that path to continue to node (ii), and the path to the right of A to still connect A and T. Unfortunately, both local algorithms can still make an incorrect choice at node (ii). Here,  the node can choose to connect two of the nodes below it, to the left, and to the right, Each of the options are valid, and so again the local algorithms choose randomly between them. In (b), the IA algorithm chooses to connect the bottom and right nodes at (ii), which does not complete the possible path between A and B. This would also be true if it connected the left and right nodes, as was done in (a). Conversely, the global algorithm in (c) makes the correct choice at both node (i), and node (ii), as it has global link information and always chooses the shortest possible path. 






==> tex/abstract.tex <==
\begin{abstract}
    As quantum key distribution becomes increasingly practical, questions of how to effectively employ it in large-scale networks and over large distances becomes increasingly important. To that end, in this work, we model the performance of the E91 entanglement based QKD protocol when operating in a network consisting of both quantum repeaters and trusted nodes. We propose a number of routing protocols for this network and compare their performance under different usage scenarios. Through our modeling, we investigate optimal placement and number of trusted nodes versus repeaters depending on device performance (e.g., quality of the repeater's measurement devices). Along the way we discover interesting lessons determining what are the important physical aspects to improve for upcoming quantum networks in order to improve secure communication rates.
\end{abstract}

==> tex/bing-command.tex <==
\usepackage{epsfig}
\usepackage{algorithm}
%\usepackage{algorithmic}
%\usepackage{algpseudocode}
%%\usepackage[figure,noline,ruled]{algorithm2e}
%%\SetKwInput{KwInput}{Inputs } \SetKwInput{KwDesc}{Description }

\newcommand{\remove}[1]{}

\newtheorem{goal}{Goal}
\newtheorem{lemma}{Lemma}
%\newtheorem{corollary}{Corollary}[section]
\newtheorem{corollary}{Corollary}
\iffalse
\newtheorem{definition}{Definition}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{Lemma}{Lemma}
%\newenvironment{proof}{{\bf Proof:}}{\hfill\rule{2mm}{2mm}}
\newcommand {\ix}{\hspace*{3mm}}
\newcommand{\1}{\mathbbm{1}}
\fi

\newcommand{\ls}[1]
   {\dimen0=\fontdimen6\the\font
    \lineskip=#1\dimen0
    \advance\lineskip.5\fontdimen5\the\font
    \advance\lineskip-\dimen0
    \lineskiplimit=.9\lineskip
    \baselineskip=\lineskip
    \advance\baselineskip\dimen0
    \normallineskip\lineskip
    \normallineskiplimit\lineskiplimit
    \normalbaselineskip\baselineskip
    \ignorespaces
   }


\newcommand{\singlefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.28\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\smsinglefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

%0.26
\newcommand{\bigsinglefig}[3]{
\begin{figure}
\centerline{
    \setlength{\epsfysize}{0.4\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\dubfigsingle}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.48\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.60\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.48\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.60\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

\newcommand{\dubfigsinglesquare}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.45\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure*}
}

%0.30
\newcommand{\tydubfigsingle}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure}
}

\iffalse
\newcommand{\tyfourfigsingle}[10]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#5}
       \newline{\small (a) #6}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.72\textwidth}
        \epsffile{\Figdir#7}
       \newline{\small (b) #8}
      \end{center}
    \end{minipage}
} \caption{#9}\label{fig:#10}
\end{figure}
}
\fi

\newcommand{\tydubfigsinglenew}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.40\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.90\textwidth}
        \setlength{\epsfysize}{0.85\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.40\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.90\textwidth}
        \setlength{\epsfysize}{0.75\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure}
}



\newcommand{\squaretydubfigsingle}[6]{
\begin{figure}
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.42\textwidth}
        \epsffile{\Figdir#1}
       \newline{\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace*{-1cm}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{1.0\textwidth}
        \setlength{\epsfysize}{0.42\textwidth}
        \epsffile{\Figdir#3}
       \newline{\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
\end{figure}
}


%
%  Triplefig.  Puts 3 figures in a 3x1 format
%
\newcommand{\triplefig}[8]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.32\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        %\setlength{\epsfxsize}{0.80\textwidth}
%        \setlength{\epsfxsize}{0.60\textwidth}
        \setlength{\epsfysize}{0.85\textwidth}
        \epsffile{\Figdir#1}\\
       {\small (a) #2}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
%        \setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.85\textwidth}
        \epsffile{\Figdir#3}\\
       {\small (b) #4}
      \end{center}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
%        \setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfysize}{0.85\textwidth}
         \epsffile{\Figdir#5}\\
       {\small (c) #6}
      \end{center}
    \end{minipage}
} \caption{#7}\label{fig:#8}
%\hrule
%\vspace*{-0.2in}
\end{figure*}
}

\newcommand{\doublefigbig}[6]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.48\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
%        \setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfxsize}{\textwidth}
        \setlength{\epsfysize}{0.85\textwidth}
        \setlength{\epsfysize}{\textwidth}
        \epsffile{\Figdir#1}\\
       {\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace{\hspace*{.5cm}}
    \begin{minipage}{0.48\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
%        \setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfxsize}{\textwidth}
        \setlength{\epsfysize}{0.85\textwidth}
        \setlength{\epsfysize}{\textwidth}
         \epsffile{\Figdir#3}\\
       {\small (b) #4}
      \end{center}
    \end{minipage}
} \caption{#5}\label{fig:#6}
%\hrule
%\vspace*{-0.2in}
\end{figure*}
}
\newcommand{\triplefigbig}[8]{
\begin{figure*}[t]
\centerline{
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfxsize}{\textwidth}
        %\setlength{\epsfxsize}{0.80\textwidth}
%        \setlength{\epsfxsize}{0.60\textwidth}
        \setlength{\epsfysize}{0.85\textwidth}
        \setlength{\epsfysize}{\textwidth}
        \epsffile{\Figdir#1}\\
       {\small (a) #2}
      \end{center}
    \end{minipage}
    \hspace{0.2in}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
%        \setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfxsize}{\textwidth}
        \setlength{\epsfysize}{0.85\textwidth}
        \setlength{\epsfysize}{\textwidth}
        \epsffile{\Figdir#3}\\
       {\small (b) #4}
      \end{center}
    \end{minipage}
    \hspace{0.2in}
    \begin{minipage}{0.30\textwidth}
      \begin{center}
        \leavevmode
%        \setlength{\epsfxsize}{0.95\textwidth}
%        \setlength{\epsfysize}{0.80\textwidth}
        \setlength{\epsfxsize}{0.85\textwidth}
        \setlength{\epsfxsize}{\textwidth}
        \setlength{\epsfysize}{0.85\textwidth}
        \setlength{\epsfysize}{\textwidth}
         \epsffile{\Figdir#5}\\
       {\small (c) #6}
      \end{center}
    \end{minipage}
} \caption{#7}\label{fig:#8}
%\hrule
%\vspace*{-0.2in}
\end{figure*}
}

\newcommand{\tysinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.30\textwidth}
        \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}


\newcommand{\longsinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.40\textwidth}
        \setlength{\epsfysize}{0.20\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}


\newcommand{\smalllongsinglefig}[3]{
\begin{figure}[t]
\centerline{
   \setlength{\epsfxsize}{0.33\textwidth}
        \setlength{\epsfysize}{0.11\textwidth}
 \epsffile{\Figdir#1}
} \caption{#2} \label{fig:#3}
\end{figure}
}

\newcommand{\Figdir}{./}


==> tex/intro.tex <==
\section{Introduction}

Quantum key distribution (QKD) allows for the establishment of information theoretically secure secret keys between two or more parties.  However, despite their great potential, these systems face several critical shortcomings when attempting to implement them in practice.  Of particular importance are improving the speed and distance of these systems.  To overcome these limitations, quantum networks are often used, consisting of \emph{trusted nodes} and, in the near future, \emph{quantum repeaters} \cite{repeater1,repeater2}.  Since quantum repeaters are still a developing technology, current QKD networks established in various metropolitan areas consist only of end-users and trusted nodes \cite{elliott2004darpa,chen2010metropolitan,peev2009secoqc,zhang2018large,sasaki2011field}.  However, progress in developing stable quantum repeaters has been accelerating of late and so it is vital to begin developing suitable routing algorithms for networks consisting of a mixture of both repeaters and trusted nodes.  Indeed, developing efficient routing algorithms to operate in this setting is vital to the future performance of such networks.

Numerous work has been done investigating the performance of quantum networks consisting only of quantum repeaters (in addition to end users) \cite{van2013path,azuma2016fundamental,hahn2019quantum,vardoyan2019stochastic,pirandola2016capacities,wallnofer2019multipartite,pirandola2019end,li2020effective}, including the development and analysis of new routing protocols specific to that scenario \cite{caleffi2017optimal,gyongyosi2017entanglement,sazim2015retrieving,pant2019routing,chakraborty2019distributed}.  Mostly, the goal of such networks is to establish end-to-end entanglement between end users (which may, then, be used for QKD for instance).  However, QKD is a more practical technology today and there are several methods to improve their performance, such as through trusted nodes.  Thus it is also important to study QKD-specific networks.  Such work has been done investigating practical QKD-specific networks consisting predominately of trusted nodes and end users \cite{dianati2008architecture,qkd-network-stack,yang2017qkd}.  However, as repeater technology progresses, the desire to move away from trusted node technology, and their inherent security concerns, will become stronger.

Thus, it is important to begin investigating near-future QKD-specific networks consisting predominately of quantum repeaters, however with a minority of trusted nodes.  Furthermore, these networks will allow for multiple paths to be established between both repeaters and trusted nodes (i.e., repeaters are not used only to extend the distance between trusted nodes, but will be an integral part of the network interior).  These are the networks we consider in this paper.  In particular, we consider a grid topology in which it is possible to establish multiple paths between Alice, Bob, and various trusted nodes though a complex network of repeaters. Our goal is to understand what routing protocols can lead to efficient key distribution rates between end users and to understand how the quality of the repeaters and the number of trusted nodes, affects the performance of this network.

In this paper, we devise and evaluate three different routing algorithms for this QKD network: one requires global state information and the other two are decentralized, distributed, algorithms requiring only local state information.
%one which requires global state information and two which are decentralized, distributed, algorithms requiring only local state information.  
We perform a rigorous evaluation, through simulations, of the performance of our algorithms in a variety of scenarios considering network size; quantum repeater quality; distance between nodes; quantity and specific location of trusted nodes; and channel noise.  Our results show that the careful design of routing algorithms is vital to establishing efficient key-distribution rates between users.  Along the way, we discover several fascinating properties of these networks which may be of great importance to operators of this future network architecture.

%OA added
%There has been much work done in analyzing the performance of QKD systems that make use of trusted nodes (CITE), and more recently there has been some analysis on the usage of quantum repeaters to extend the range of quantum networks (CITE). 

%To those ends, in this work we introduce a model for future QKD networks of this form, in which the goal is to utilize both quantum repeaters and trusted nodes to establish as large a secret key as possible between two users, Alice and Bob, in a given time frame or number of communication cycles. We introduce three new protocols to be used by the network to route entanglement generation, and analyze the performance of the network under each one for a number of different network scenarios and trusted node configurations. We find that the choice of protocol can have a large impact on what key rates the network can achieve, even comparable to the impact that the addition of trusted nodes can have. We also discover some interesting guidelines for optimal performance based on device characteristics which may be valuable to future practitioners of these near future networks. 


%In this paper we develop new routing algorithms and analyze, through simulations, their performance in a large-scale QKD network consisting of both trusted nodes and quantum repeaters.  The goal of this network is to serve two users $A$ and $B$, allowing them to establish as large a secret key as possible within a given amount of time or number of communication cycles.  We consider a near-future network consisting of both trusted nodes and quantum repeaters, and propose three different routing algorithms for this scenario.  We evaluate our routing algorithms in a variety of network configurations where we alter the number and location of trusted node units. We also discover some interesting guidelines for optimal performance based on device characteristics which may be valuable to future practitioners of these near future networks.
%\bing{Is it fair to say that the main contribution of our paper is design and evaluate routing algorithms in a quantum network with both quantum repeaters and trusted nodes? Existing studies either consider networks with quantum repeaters but no trusted nodes, or quantum networks with trusted nodes but no repeaters. In addition, our paper considers a more complex grid network topology (instead of line-type network),  and we show indeed that the routing algorithm can impact the resulting key generation results significantly. It will be good to highlight the main challenges/questions and opportunities in a grid network with both quantum repeaters and trusted nodes. Challenges/questions: repeaters are not perfect (decoherence, imperfect BSM), where to place trusted nodes, benefits of more trusted nodes? Opportunities: shorter distance between end users and trusted nodes, multipath is possible?} 

\subsection{Quantum Key Distribution}
Quantum key distribution (QKD) protocols operate in two stages: In the \emph{quantum communication stage}, users Alice and Bob use the quantum channel and the authenticated classical channel to attempt to establish a \emph{raw key} which is a classical bit string that is partially correlated (there may be errors in the quantum channel leading to errors in the raw key) and partially secret (an adversary may have some information on the raw key).  Since this raw key cannot be used directly for cryptographic purposes, a second, purely classical, stage is performed, running an error correction protocol (leaking additional information to an adversary) followed by privacy amplification, which leads to the final secret key.  An important metric in any QKD protocol is the protocol's \emph{key-rate} defined to be the ratio of secret key bits to the size of the raw key.  For a general survey of QKD protocols, the reader is referred to \cite{QKD-survey-old,QKD-Survey}.

In this work, we are interested in the theoretical performance of a network of QKD systems.  As such, we consider ideal single-qubit sources (though potentially there is loss due to the fiber channel connecting nodes).  Furthermore, we do not consider finite key effects \cite{scarani2008quantum} or imperfect sampling, in an attempt to understand the theoretical behavior of the network.  Under this setting, the key-rate of the E91 \cite{QKD-E91} protocol, which we adopt as the QKD protocol used in our network, is found to be \cite{QKD-BB84-rate1,QKD-renner-keyrate}: $\texttt{rate} = 1-2h(Q)$, where $Q$ is the bit error rate in the raw key and $h(\cdot)$ is the binary entropy function.  Note that, if we did not assume single-qubit sources and, instead, weak coherent sources, we would need to use an alternative key-rate expression or, perhaps, the decoy state BB84 protocol \cite{lo2005decoy}; these are interesting issues we leave as future work.

Point-to-point QKD systems are often implemented over fiber channels (though free-space operation is also possible if one has direct line of sight).  One limitation to QKD protocols is their intolerance to qubit loss \cite{pirandola2017fundamental,QKD-Survey}; since loss over a fiber channel scales exponentially with distance, this is particularly problematic for ground operation.  To overcome this, one may use \emph{quantum repeaters} \cite{repeater1,repeater2} and \emph{trusted nodes}.  Both systems are placed between users, thus halving the total distance a qubit is required to travel; furthermore, multiple such nodes may be chained together thus further decreasing the distance.  Quantum repeaters utilize entanglement swapping to produce a shared entangled bit between two users.  Trusted nodes act as users in a QKD protocol, establishing a key $k_{AT}$ with Alice and a second, independent key, $k_{TB}$ with Bob.  The trusted node then sends to $B$ (using an authenticated classical channel) the value $k_{AT}\oplus k_{TB}$, where $\oplus$ is the bit-wise XOR.  This allows Alice and Bob to share a classical key, though the trusted node also shares this key.

The advantage to quantum repeaters is that the final key $A$ and $B$ produce is independent of the repeater's knowledge.  That is, if a repeater is controlled by an adversary, it cannot learn the final secret key.  However, the technology for repeaters requires short-term quantum memories which is a difficult engineering challenge (though the technology is rapidly advancing).  Trusted nodes have the advantage of simplicity as they are no different in technology than Alice or Bob.  However, they must remain trusted and safe from an adversary as they do have full knowledge of the secret key.

%% FOR INTRO: Currently, QKD networks typically rely on trusted node technology (CITE).  However, as repeaters are advancing, it is important to begin considering complex networks consisting of both repeaters and trusted nodes (where multiple paths are allowed for both repeaters and trusted nodes), and the challenges therein.  This is the form of network we consider in this work.


\subsection{Related Work}
There has been recent research in analyzing routing protocols, along with the general behavior and performance, of quantum networks consisting of end-users and quantum repeaters, but no trusted nodes; see for instance \cite{van2013path,azuma2016fundamental,caleffi2017optimal,gyongyosi2017entanglement,hahn2019quantum,pant2019routing,vardoyan2019stochastic,chakraborty2019distributed,pirandola2016capacities,wallnofer2019multipartite,pirandola2019end} with \cite{caleffi2017optimal,gyongyosi2017entanglement,pant2019routing,chakraborty2019distributed} giving particular focus on specific routing protocols for certain network topologies in generating shared entanglement between users, which is a stronger resource than QKD. However, QKD is, currently, a more practical and mature technology and, furthermore, there are numerous methods of improving the performance (speed and distance) of these systems that are unavailable to entanglement generation networks, namely the use of trusted nodes.  Thus, while routing protocols designed for an entanglement-generation quantum internet can be used also for QKD, more efficient systems may exist and, furthermore, solutions incorporating both trusted nodes and repeaters are vital for near-term deployment of this technology and are the networks we consider in this work.

Early work on QKD-specific networks focused on algorithms for optical-based switching networks \cite{toliver2003experimental}.  Such networks were used in practice, for instance the 2004 DARPA network in the Boston area \cite{elliott2004darpa,elliott2005current} and the 2009 network in Hefei \cite{chen2010metropolitan}, utilized such an architecture (the Hefei network also utilized trusted nodes).  These networks consisted of end-users and optical switches allowing users to route qubits to each other.

A more capable QKD network consists of end-users and trusted nodes and is the most common of network architectures for practical QKD networks in operation today such as the SECOQC network in Vienna \cite{peev2009secoqc}, the previously mentioned Hefei network \cite{chen2010metropolitan}, the Tokyo QKD network \cite{sasaki2011field} and the Beijing-Shanghai network \cite{zhang2018large}.  In terms of routing algorithms, the Vienna network used a variant of the OSPF routing algorithm \cite{dianati2008architecture}.  In \cite{tanizawa2016routing}, required functionalities of a QKD network routing algorithm were described for this form of network and a routing protocol was proposed, while \cite{yang2017qkd} began constructing routing protocols for larger scale networks evaluated through simulations. A novel quality of service model for these networks, and new routing protocols, were introduced in \cite{mehic2019novel}.  A complete QKD network stack for such networks was proposed in \cite{qkd-network-stack}, along with advanced routing functionalities through trusted nodes taking into account channel performance and key-rate demands, while in \cite{li2020mathematical}, a mathematical model was proposed for analyzing such trusted-node QKD networks.

The severe limitation to trusted nodes is that, as their name implies, they must be trusted.  Indeed, a trusted node is fully aware of the secret key which $A$ and $B$ distill (multi-path routing is one counter-measure to this, though still imperfect).  An advancement from this would be the use of quantum repeaters.  However, while the technology for these is advancing rapidly, it is more likely that in the near-future, any QKD network will consist of both repeaters and trusted nodes.  Thus, developing new and efficient routing algorithms specific for this network technology, is vital.  In this work, we consider networks that consist of a majority of repeaters with a minority of trusted nodes, attempting to discover optimal routing protocols for this scenario and to understand the behavior of such a network.  Note that in \cite{qkd-network-stack}, the use of quantum repeaters in a chain to link together different trusted nodes was considered an option; here, however, we are considering more complex networks of repeaters, allowing for potential multi-path routing options between both trusted nodes and multiple repeaters. 
%\OA{Interestingly it seems like the takeaway of our work is that there is no getting away from trusted nodes, even with perfect quantum repeaters. (as long as there is decoherence, though i have been wondering (for the future) if our assumption that channel decoherence doesn't scale with length is practical. if it wasn't, then perfect repeaters could probably replace trusted nodes.}


==> tex/model-simulator.tex <==
\section{Model and Simulator}\label{sec:model}

In this work we consider a grid network consisting of $N\times N$ nodes with each node connected to at most four others, their immediate neighbors up, down, left, and right.  These connections represent fiber links allowing for the direct transmission of qubits between neighboring nodes only.  We assume a classical communication network allowing any pair of nodes to send classical messages.  We do not assume this communication is secret; however for all user and trusted node communication we do assume it is authenticated.  Each node in this network may be either a User (Alice or Bob); a Trusted Node; or a Quantum Repeater.  We place Alice at the lower-left corner of the network and Bob in the upper-right (thus, these users have only two neighbors they are connected to).  Later, we will simulate alternative numbers and locations of the trusted nodes; however, predominately the other nodes will consist of quantum repeaters in contrast to current day QKD networks.

\triplefig{stage1.pdf}{Initial network}{stage2.pdf}{Stage 1}{stage3.pdf}{Stage 2}{(a) The initial network of a $5\times5$ grid, with a central trusted node ($T$) between Alice ($A$) and Bob ($B$). (b) A possible network configuration after stage 1, in which some nodes succeed in establishing a shared state of the form in Equation (\ref{eq:shared-state0}) with their neighbors over the fiber channels and some do not. 
%Note that there are a number of possible paths between A, B and T. 
(c) Successful entanglement chaining and routing (depicted as the ``internal links'' at repeaters) as discussed in Stage 2. In this graph, routing has resulted in end-to-end paths being created between each pair of $A$, $B$ and $T$. These routes are successful only if every Bell state measurement along the path succeeds. Furthermore, the probability of decoherence increases with the path length in our model as discussed; thus minimizing the path lengths through effective routing algorithms and trusted nodes is advantageous.  See also Figure \ref{fig:guide}.}{stages1-3}

%%intra-repeater connections

\begin{figure}
    \centering
    \includegraphics{sideguide.pdf}
    \caption{A legend for our network diagrams. Left: (a) denotes a node in the network, specifically a repeater with 4 (b) connection terminals from which entangled photons are sent and received over (c) fiber optic connections between other repeaters and (d) trusted nodes. Right: an entangled channel (e) connecting multiple trusted nodes through intra-node entanglement (f).}
    \label{fig:guide}
\end{figure}

Users and trusted nodes perform the E91 QKD protocol.  For notation, we assume there are $n$ trusted nodes denoted $T_1, \ldots, T_n$.  We label Alice as $T_0$ and Bob as $T_{n+1}$.  For every pair of users and trusted nodes there exists a private raw-key pool; that is, for every $i,j \in \{0,\cdots, n+1\}$, with $i < j$, there exists a buffer $\rawkey_{i,j}$, storing the raw key shared between nodes $T_i$ and $T_j$.  Note that repeaters do not have key buffers.  As we are using the entanglement based E91 protocol, the first goal of the network is to establish joint entanglement between these pairs of nodes $T_i$ and $T_j$, ideally the Bell state $\ket{\Phi^+} = \frac{1}{\sqrt{2}}(\ket{00} + \ket{11})$.  This resource may be used to establish a secret key between users.

The quantum network we analyze operates in {\em rounds}, each round consisting of {\em three primary stages} (see examples in Figures \ref{fig:stages1-3} and \ref{fig:guide}).  The first stage, and part of the second stage, are standard in repeater-only quantum networks (see \cite{pant2019routing,chakraborty2019distributed}). As mentioned, nodes have at most four inputs into them (since the two users are at the corner of grid, they each only have two inputs); we assume that nodes have the capability of storing a single qubit in short-term memory for each of these inputs, through one complete round.  After the round is complete, any qubits not measured, are discarded.  That is, the memory capabilities of nodes are not sufficient to store a qubit through two or more rounds in our network.  Note that users in our network have the fewest demands on quantum memory.

In the first stage, adjacent nodes attempt to share an entangled pair, in particular the Bell state $\ket{\Phi^+}$, with one particle remaining at a local node and the other being transmitted to an adjacent node.  Due to fiber loss, this succeeds with a certain probability $p = 10^{-\alpha L/10}$ where $\alpha$ is the fiber attenuation coefficient (we use $\alpha = .15$ in our later simulations).  Furthermore, even if successful, the entangled pair may not be a Bell state $\ket{\Phi^+}$ but instead will, with probability $D$, depolarize and become completely mixed.  Ultimately, after this first stage, adjacent nodes $u$ and $v$ will either not have any qubit in their short-term memory (with probability $1-p$) or, with probability $p$, they will share a quantum state of the form:
\begin{equation}\label{eq:shared-state0}
\rho_{u,v} = (1-D)\kb{\Phi^+} + D \cdot \frac{I}{4},
\end{equation}
where $I$ is the identity operator on two qubits.  Note this $D$ may be used to model channel noise along with noise internal to the quantum memory of the repeater.  As is standard in repeater-network analyses \cite{pant2019routing,chakraborty2019distributed}, we assume that nodes are able to determine whether a qubit has arrived in their short-term quantum memory or if it is a vacuum.

In the second stage, a routing protocol, to be discussed (see Section~\ref{sec:routing}), is performed to decide how to %optimally 
effectively route entanglement between nodes $T_i$ and $T_j$ for $i \ne j$.  This routing protocol can take into account whether nodes have a qubit in their short-term memory.  The goal of this stage, and in particular the routing algorithm, is to determine a set of paths, the end-points of which are either users or trusted nodes, while the interior nodes of each path are quantum repeaters.  Given these paths, the quantum repeaters will perform entanglement swapping operations on the qubits that are locally held in their short-term memory, which, if successful, create ``virtual'' entangled links between the end-points of each path.
%attempting to create an end-to-end entangled pair between the end-points of each path.  
The entanglement swapping operations at the repeaters, which themselves consist of Bell measurements, succeed only with a certain probability that we denote as $B$.  We assume the network is able to determine whether a successful entanglement swapping occurred or not.  Thus, at the end of this stage, end-nodes $T_i$ and $T_j$ on each path can determine whether the network was successful in creating an end-to-end  path between these nodes.  Note that they cannot tell if the state they share is the correct Bell state $\ket{\Phi^+}$ or the completely mixed state $I/4$ due to depolarization.  At this point, repeaters are no longer needed until the next round, and users and trusted nodes share a state of the form in Equation (\ref{eq:shared-state}), where the probabilities of the mixed state depend on $D$ and the path length -- in particular, on a path consisting of $k$ interior nodes, the shared state will either be:
\begin{equation}\label{eq:shared-state}
\rho_{T_iT_j} = (1-D)^{k+1}\kb{\phi^+} + (1-[1-D]^{k+1})\cdot\frac{I}{4},
\end{equation}
or a vacuum if one or more repeaters failed in their entanglement swapping operation.

Finally, in the third stage, all pairs $T_i$ and $T_j$ of users and trusted nodes which have a shared state, and not a vacuum, attempt to distill a raw-key bit using the E91 QKD protocol.  If successful (which depends on users choosing the correct basis, and as such it is successful with probability $1/2$), the key-bit is added to a local raw key-pool for those users $\rawkey_{i,j}$.  Any qubit that was not measured by now is discarded and the network repeats at stage 1, attempting to establish fresh entangled pairs between adjacent nodes.  Refer to Figures \ref{fig:stages1-3} and \ref{fig:guide}.

We wrote a custom simulator to simulate the behavior of this network and these three stages.  This simulator maintains a raw-key pool $\rawkey_{i,j}$ between each pair of users $T_i$ and $T_j$ as would be done in an actual operation of this network.  In practice, nodes $T_i$ and $T_j$ will, once the length of the raw key in $\rawkey_{i,j}$ is sufficiently large, perform error correction and privacy amplification, leading to a secret key of size $|\secretkey_{i,j}|$.  In our simulations, we are interested in the theoretical performance of this network, and so we only do this process once at the end of the simulation and set $|\secretkey_{i,j}| = |\rawkey_{i,j}|\cdot (1-2h(Q))$ where $Q$ is the error in the raw key pool $\rawkey_{i,j}$ and where $h(x)=x\log(x)-(1-x)\log(1-x)$ is the binary entropy function. Again, as we are only interested in theoretical behavior, we compute $Q$ based on the actual simulator data; in practice $Q$ may be estimated by sampling from $\rawkey_{i,j}$.

Of course, the ultimate goal of the network is to maximize the secret key pool between Alice and Bob (i.e., $T_0$ and $T_{n+1}$).  If $n=0$ (i.e., there is no trusted node), at this point, we are done.  However for $n\ge 1$, a final key-routing process is required of the trusted nodes who must attempt to ``push'' a maximal amount of key material to Alice and Bob.  For $n=1$, this is trivial: $T_1$ will simply broadcast $\secretkey_{0,1}\oplus \secretkey_{1,2}$ (here, $T_0$ is Alice and $T_2$ is Bob); if they are not of equal length, then only the left-portion is broadcast.  Alice and Bob already have a secret key of size $|\secretkey_{0,2}|$ before this process.  Thus, finally, they end up with a secret key of total size $|\secretkey_{0,2}| + \min(|\secretkey_{0,1}|, |\secretkey_{1,2}|)$.  When $n > 1$ the situation is more complicated; in this work we use the max-flow algorithm to determine how many additional bits are appended to $\secretkey_{0,n+1}$.  Note that, at the end, not all key bits in trusted node pools may be usable if there is an insufficient amount of key material in ``matching'' nodes.  Later, when we evaluate performance of our routing protocols, we will look at the key-rate of the network, namely the size of the final secret key between Alice and Bob (after the trusted nodes perform this final key-routing process) divided by the total number of network rounds.  



==> tex/more-trusted-node.tex <==
\subsection{Multiple Trusted Nodes} \label{sec:more-trusted-nodes}

%\bigsinglefig{TNs.pdf}{A $7\times7$ network with 3 different placements of the two trusted nodes. The nodes labeled with $A$ and $B$ are Alice and Bob in each type of placement; the two nodes labeled with $C$ are the trusted nodes in the {\em corner} configuration; the two nodes labeled with $D$ are the trusted nodes in the {\em diagonal} configuration; and  the two nodes labeled with $R$ are the two trusted nodes in the {\em asymmetric} configuration.}{TNPlacement}

\singlefig{TNs.pdf}{A $7\times7$ network with 3 different ways of placing the two trusted nodes. The nodes labeled with $A$ and $B$ are Alice and Bob in each type of placement; the two nodes labeled with $C$ are the trusted nodes in the {\em corner} placement; the two nodes labeled with $D$ are the trusted nodes in the {\em diagonal} placement; and  the two nodes labeled with $R$ are the two trusted nodes in the {\em asymmetric} placement.}{TNPlacement}


%\triplefigbig{figs/2TN_g.png}{Global}{figs/2TN_IA.png}{Intersection Avoidant}{figs/2TN_NIA.png}{Non-Intersection Avoidant}{These charts are obtained from simulations on a 7x7 grid with $L=1$ and $B=.85$. The 2-Diagonal data is the result of placing two trusted nodes along the diagonal between Alice and Bob, such that the distance between the two trusted nodes is equal to the distance between Alice/Bob and the closest trusted node to each of them. The 2-Asymmetric data is the result of having a trusted node in the center of the network, with one additional trusted node one position closer to Alice on the diagonal. The 2-Corner data comes from a trusted node configuration with a trusted node at opposite corners of the grid. Finally, the 1-Central configuration has a single trusted node at the center of the graph. Each chart shows the effect of the decoherence rate on the key rate for a specific routing algorithm.}{2TNGraphs}

\triplefigbig{figs/2TN_g.pdf}{Global}{figs/2TN_IA.pdf}{Intersection Avoidant}{figs/2TN_NIA.pdf}{Non-Intersection Avoidant}{Key rate versus the decoherence rate for the three routing algorithms in a $7\times7$ grid with $L=1$ km and $B=.85$. We consider the No TN case, the Central TN case, and the 2 TN cases in which there are two trusted nodes in the network, following corner, diagonal or asymmetric placements. }{2TNGraphs}

\tydubfigsingle{figs/S_fixed_global.pdf}{Global}{figs/S_fixed_IA.pdf}{Intersection Avoidant}{Key rate versus the network size for the global and IA routing algorithms for a 10 km $\times$ 10 km network grid where the fiber length between each node decreases as the network size increases. Notably, we see some non-monotonicity as the diagonal configuration does not operate effectively at grid sizes that are not of the form $3x+1$ for some integer $x$, and the central case does not operate effectively at even grid sizes such as 10x10. }{FixedLength}

\tydubfigsingle{figs/B_all2E_global}{Global}{figs/B_all2E_IA}{Intersection Avoidant}{Key rate versus the BSM Success rate for the global and IA routing algorithms in a $7\times7$ grid with $L=1$ km and $D=.02$. We consider the no TN case, the central TN case, and the 2 TN cases in which there are two trusted nodes in the network, following corner, diagonal or asymmetric placements.}{2TNGraphsB}



We now consider having two trusted nodes in the network. Specifically, we investigate three methods of placing these two trusted nodes, referred to as {\em corner}, {\em diagonal}, and {\em asymmetric} placements. In the corner placement, the two trusted nodes are located at the two opposite corners of the graph (distinct from Alice and Bob's corners); in the diagonal placement, the two trusted nodes are placed evenly along the diagonal between Alice and Bob; in the asymmetric placement, one trusted node is located in the center, while the other is located one node along the diagonal closer to Alice. Fig.~\ref{fig:TNPlacement} illustrates the above three types of placement for a $7\times7$ grid (we use a $7\times7$ instead of a $5\times5$ grid as the diagonal placement only performs optimally for grid size $N =3x+1$ for some integer $x$). 


%\WK{These figures are out of order 10, then 8,9} 
Figures~\ref{fig:2TNGraphs}(a) through (c) plot the key rate as the decoherence rate increases for each of the above types of placement for the global, IA and NIA routing algorithms, respectively. For comparison, in each figure, the results with a single trusted node placed in the center and no trusted node are also plotted in the figure. We see that for the global routing algorithm (see Fig.~\ref{fig:2TNGraphs}(a)), the diagonal placement outperforms the other four cases (i.e., corner and asymmetric placement of two trusted nodes, as well as no trusted node and placing a single trusted node in the center) by a large margin. 

The clustering of the non-diagonal configurations we attribute to two separate reasons. First, consider that in the central configuration, an optimal pathing results in two channels connecting Alice to the trusted node, and two more connecting the trusted node to Bob. Importantly, these channels will consist of 6 edges each. In the corner configuration, an optimal pathing results in one channel between Alice and each of the two trusted nodes, and likewise from Bob to the trusted nodes. Again, these channels will consist of 6 edges each. As a result, at least in the global case, the likelihood that these paths exist, that the channels are successfully established and that the entanglement remains coherent are all equivalent. It stands to reason then, and the data reflects that reasoning, that the corner configuration and the central configuration are equivalent, in terms of performance. In the other case, it is the asymmetry that causes the equality. Although the second trusted node does result in Alice and the central trusted node sharing a larger key, the central trusted node and Bob establish no more key-bits than if the second trusted node did not exist. As a result, in the final routing of key material, the overall capacity between Alice and Bob remains unchanged, and so the additional key-bits that Alice and the trusted node were able to establish go unused. Finally, the over-performance of the diagonal configuration is a result, as one would expect, from the further segmentation of the $7 \times 7$ network into 3 distinct sub-networks: between Alice and the first trusted node; the first and second trusted nodes; and finally the second trusted node and Bob. As shown in the figure, this additional trusted node can increase our key rate by almost a factor of 1.5 over the central trusted node configuration. 

We repeat the above investigation for the IA algorithm (see Fig.~\ref{fig:2TNGraphs}(b)). Again, we see that the diagonal placement outperforms the others, and that the performance of the corner placement of two trusted nodes is very similar to that when placing a single trusted node in the center. We also see, however, that the redundant trusted node in the asymmetric case results in a large detriment to the key rate, dropping it almost a full .3 key-bits/round. This is likely due to the greedy nature of the routing algorithm -- having an additional node complicates the decision process of the repeaters near both trusted nodes, potentially wasting edges that otherwise could have been utilized in a more effective manner.

The differences in the performance of the different types of placement are even more dramatic for the NIA algorithm in Fig.~\ref{fig:2TNGraphs}(c). For each configuration we see a significant drop in performance, except for the corner placement, which remains relatively consistent with its performance in the other algorithms. This difference can be explained by the fact that that the NIA algorithm does not generally struggle with intersecting paths in the corner case, as the optimal paths themselves tend not to contain many right angles. The effect of this is so great, in fact, that at lower error rates the corner configuration in fact outperforms the diagonal configuration, until the shorter hop-length of the channels in the diagonal configuration becomes the dominating factor in determining key rate. 

%\OA{Bing, does this make more sense? (comment was: )bing\{Are you increasing the distance? This is for a fixed 10km x 10km network, right?\}}

As physical distance between Alice and Bob increases, one might think that there is benefit to be had by adding additional repeaters and decreasing the distance between nodes themselves. We investigate whether or not this is feasible in Fig.~\ref{fig:FixedLength} in which the physical distance the network spans is fixed at $10$ km $\times$ $10$ km, while the number of nodes in the grid is increased (this is in contrast to our other simulations where the total width of the network was not fixed, but instead, the length and width are both $(N-1)\cdot L$ km). What we see is that the tendency for BSM failure chance and decoherence probability to increase as path sizes increase puts a damper on any benefit that can be achieved through this method. In some scenarios it is likely that there are trade-offs that can be made, depending on the target distance between Alice and Bob, BSM success probabilities, and decoherence probabilities, but evidently there are limitations inherent to trying to augment the key rate using this method. 

It is clear, however, that this limitation can be alleviated in part by the addition of trusted nodes. As can be seen in Fig.~\ref{fig:FixedLength}, while the key rate of each configuration decreases as the size increases, even as the fiber length decreases, additional trusted nodes remain effective in boosting the key rate. As a result, it is still possible to increase network size to alleviate fiber length concerns, as long as the number of trusted nodes is also increased.  Additionally, 
%showcased by these charts is 
Fig.~\ref{fig:FixedLength} showcases the way in which non-optimal grid sizes affect key rate for the different TN configurations. Namely, we see that the key rate of the diagonal configuration actually increases between $N=5$ and $N=7$, or $N=9$ and $N=10$, as we move from grid sizes not of the form $3x+1$ to grid sizes of that form. We see the same for the central configuration at the even grid size of $N=10$, where the node is placed slightly off center, and as such actually increases at $N=11$. 

Finally, in Fig.~\ref{fig:2TNGraphsB} we consider the performance of the global and IA algorithms on a number of TN configurations as the BSM success probability increases. Again, we see that the general trend is the same between the global and IA algorithms, with the global algorithm outperforming the IA algorithm in each configuration, and especially the asymmetric case. In the diagonal configuration, with perfect quantum repeaters (i.e. $B=1$), both are able to achieve a key rate of more than .45 key-bits/round with 2 TN in the diagonal configuration, and with 1 TN in the center, the IA algorithm and global algorithms achieve key rates of .3 and .33 key-bits/round, respectively. 
%These charts in particular are notable, because they 
The above results are notable, because they give some sense of the trends we might expect to see as quantum repeater technology advances. They also show the great benefit to using trusted nodes, even with perfect, ideal, repeaters.




%%wb, 5/14/2020, older version
\iffalse 
one with the two trusted nodes located at the two opposite corners of the graph (distinct from Alice and Bob's corners), one with the two trusted nodes distributed evenly along the diagonal between Alice and Bob, and one with one trusted node located at the center, and the other located one node along the diagonal closer to Alice. We refer to the above three types of placements as the {\em corner}, {\em diagonal}, and {\em asymmetric} configurations, as illustrated in Fig.~\ref{fig:TNPlacement} for a $7\times7$ grid (we use a $7\times7$ instead of a $5\times5$ grid since the diagonal configuration only performs optimally for grid size $N =3x+1$ for some integer $x$). Fig.~\ref{fig:2TNGraphs} plots the key rate under the these three placements of two trusted nodes. For comparison, the results with a single trusted node placed in the center are also plotted in the figure. 
%We show the effect that decoherence rate has on the performance of these configurations, alongside the performance for a single, central trusted node, for each of the algorithms in Fig.~\ref{fig:2TNGraphs}. We note that in order to equally distribute two trusted nodes along the diagonal, we moved the network size from 5x5 to 7x7, and in fact the diagonal configuration only performs optimally at grid sizes of NxN where N $=3x+1$ for some $x$.  
 


What we find is that, in the global case (as shown in Fig.~\ref{fig:2TNGraphs}(a), the corner, central, and asymmetric configurations perform at essentially the same level, while the diagonal configuration outperforms the others by a large margin. The clustering of the non-diagonal configurations we attribute to two separate reasons. First, consider that in the central configuration, an optimal pathing results in two channels connection Alice to the trusted node, and two more connecting the trusted node to Bob. Importantly, these channels will consist of 6 edges each. In the corner configuration, an optimal pathing results in one channel between Alice and each of the two trusted nodes, and likewise from Bob to the trusted nodes. Again, these channels will consist of 6 edges each. As a result, at least in the global case, the likelihood that these paths exist, that the channels are successfully established and that the entanglement remains coherent are all equivalent. It stands to reason then, and the data reflects that reasoning, that the corner configuration and the central configuration are equivalent, in terms of performance. In the other case, it is the asymmetry that causes the equality. Although the second trusted node does result in Alice and the central trusted node to share a larger key, the central trusted node and Bob establish no more key-bits than if the second trusted node did not exist. As a result, in the final routing of key material, the overall capacity between Alice and Bob remains unchanged, and so the additional key-bits that Alice and the trusted node were able to establish go unused. Finally, the over-performance of the diagonal configuration is a result, as one would expect, from the further segmentation of the 7x7 network into 3 distinct sub-network between Alice and the first trusted node, the first and second trusted nodes, and the second trusted node and Bob. As shown in the figure, this additional trusted node can increase our key rate by almost a factor of 1.5 over the central trusted node configuration. 

In the second figure, Fig. ~\ref{fig:2TNGraphs}(b), we repeat this investigation for the Intersection Avoidant algorithm. again we see that the diagonal configuration outperforms the others, and that the corner and central configurations are equivalent. We also see, however, that the redundant trusted node in the asymmetric case results in a large detriment to the key rate, dropping it almost a full .3 key-bits/round. This is likely due to the additional node complicating the decision of repeaters near both nodes, potentially wasting edges that otherwise could have been utilized in an effective manner.

The differences in performance are even more stark when we look at the Non-Intersection Avoidant algorithm in the third chart, Fig~\ref{fig:2TNGraphs}(c). For each configuration we see a significant drop in performance, save for the corner configuration which remains relatively consistent. This difference can be explained by the fact that that the NIA algorithm does not generally struggle with intersecting paths in the corner case, as the optimal paths themselves tend not to contain many right angles. The effect of this is so great, in fact, that at lower error rates the corner configuration in fact outperforms the diagonal configuration, until the shorter hop-length of the channels in the diagonal configuration becomes the dominating factor in determining key rate. 
\fi




% To understand how additional trusted nodes can affect the key rate, we investigated a number of different trusted node configurations. As can be seen in  Fig.~\ref{fig:2TNGraphs}, placing two trusted nodes along the diagonal of the network, rather than one, can further divide the network into shorter, more segments, leading to higher key rates and robustness. At the same time, we see that placing two trusted nodes at the corners of the grid does not lead to an advantage over a single, central node, and indeed the two cases, for the Global and IA algorithms, seem to be equivalent. For the non-global algorithms, we also see that the addition of a redundant trusted node, can in fact greatly reduce the key rate, rather than enhance it.
% We found that the "effective" usage of two trusted nodes was to place them along the diagonal, dividing the diagonal into three equal segments. On a 5x5 grid, this could not be done, so we here we instead compare the performance of various trusted node configurations on a 7x7 grid. In fact, this division can only occur on grids of size $N$x$N$, where $N$ is one more than a multiple of 3. At other grid sizes the diagonal configuration still achieves higher key rates than when there is a single trusted node, but there is not a monotonic relation between key rate and grid size.




==> tex/old-sim.tex <==
\subsection{Simulator}
\begin{figure}
    \centering
    \includegraphics{sideguide.pdf}
    \caption{A legend for Figure \#\ref{fig:stages1-3}. (a) denotes a node in the network, specifically a repeater with 4 (b) connection terminals from which entangled photons are sent and received over (c) fiber optic connections between other repeaters and (d) trusted nodes. Below the line, an entangled channel (e) connecting multiple trusted nodes through intra-node entanglement (f)}
    \label{fig:guide}
\end{figure}

%%wb, 4/20/20, put three figures in stages 1-3 side by side 
\triplefig{stage1.pdf}{Stage 0}{stage2.pdf}{Stage 1}{stage3.pdf}{Stage 2}{(a) The initial network, in a 5x5 grid, with a central trusted node (T) between Alice (A) and Bob (B), as discussed in stage 0. (b) A possible network configuration after stage 1, in which some nodes succeed in establishing a shared EPR pair with their neighbors over the fiber channels and some do not. Note that there are a number of possible paths between A, B and T. (c) Successful entanglement chaining and routing (depicted as the intra-repeater connections) as discussed in stage 2. In this graph, routing has resulted in a channel being created between each pair of A, B and T. These routes are successful and coherent only if every bell state measurement along the path succeeds, and if no decohering occurs in the path, so minimizing the path lengths with effective routing algorithms and trusted node utilization is advantageous. For the purposes of this diagram we condition on the channels remaining coherent, but in practice any could have become decoherent.}{stages1-3}
To analyze the behavior of the QKD network we envision and to evaluate the performance of the various routing protocols we construct later, we wrote a custom simulator.  This simulator, following an initialization stage, operates in four steps, which each  take in as input the state of the network graph at the end of the state prior and outputting the resulting, evolved graph. \par
\textbf{0. Initialization:}
Consider an $N\times N$ (for an odd $N$) network graph with some number of trusted nodes and Alice and Bob at opposite corners of the network, Such a network begins in the state $G = \{V,E\}$ where $V = \{0,1, \dotso,N^2-2, N^2-1\}$ with Alice at node $A=0$ and Bob at node $B = N^2-1$, and trusted nodes $T \subseteq V$. Finally, without loss of generality we consider a grid network in which the nodes are ordered increasing from left to right and bottom to top, and so we have $E$ defined in the natural way. We show the steps describing the evolution of this graph in the following section, as well as the evolution of this example graph in Figs.~\ref{fig:stages1-3} and \ref{fig:stage5}, with a key provided in Fig.~\ref{fig:guide}. \par
\textbf{1. Entanglement Generation:} In the initial phase, each node attempts to share one half of a  Einstein–Podolsky–Rosen (EPR) \cite{EPR} pair with its neighbors over the fiber channel. The photon pair is successfully transmitted and received with probability $10^{-\alpha L/10}$ \cite{transmittance} where $\alpha$, also a characteristic of the network, is the transmittance of the fiber channel. As such the network evolves to $G_1 = \{V, E_1\}$ where $E_1 = \{(u,v) \forall (u,v) \in E  \; |\;  S(u,v) \}$  \OA{what is set notation for random sets?}, where $S(u,v)$ is a random binary function that returns true for any edge with probability $10^{-\alpha L/10}.$ \par
\textbf{2. Routing and Entanglement Chaining: } With the evolved network graph, the repeater nodes utilize a routing algorithm (we will discuss a number of candidate algorithms in the following section) to determine, at each repeater, which neighbors should be connected by entanglement. The routing algorithm, $R1$, takes $G_1$ as input and outputs $P = \{p_i\}_{i=0}^n$ where $p_i = (r_0^i, r_1^i, \dotso, r_{m_i}^i)$ describe paths originating from and ending at Alice, Bob, or a trusted node through a path of $m-2$ entanglement connected quantum repeaters. The quantum repeaters then use this pathing information and conduct bell state measurements on the photons they hold that are entangled with photons at the nodes before and after them in a path \bing{this sentence is a bit long; can we rephrase by using the notation?}, succeeding with probability $B$ and becoming decoherent with probability $D$. As a result of this action, the network evolves and is compromised of Alice, Bob, trusted nodes, and shared entanglement (which with some probability has decohered) between those parties. Specifically, we have $G_2 = \{V_2, E_2\}$ where $V_2 = T\cup \{A,B\}$ and $E_2 = \{(r_0^i,r_{m_i}^i,F(p_i)) \; \forall p_i \in P\}$ where $F(p_i)$ is a random binary function that decides whether or not the entangled channel has fidelity. Fidelity is maintained with probability $(1-d)^{m_i-2}$, as it must be the case that at each of the $m_i-2$ intermediate nodes, the bell state measurement did not fail. We note that as there can be multiple (up to two) paths between the same pair of entities, the elements in $E_2$ are not necessarily unique. \par
\textbf{3. Quantum Key Distribution:} In this stage, the entities in $G_2$ attempt to use the quantum channels established between them to conduct a round of an entanglement based QKD protocol --- in our case, E91. Here we will  introduce a secondary network structure, with weighted edges connecting Alice, Bob, and trusted nodes with weights representing the amount of key material shared between nodes. The edges additionally have associated with them a bit string, with length equal to their weight, representing whether there is a correlation in each bit of key material (though the value of the bits themselves, for the purpose of our simulation, is irrelevant). This graph, at the start of the protocol, is initialized to $G_3 = \{V_2, E_3\}$ where $E_3 = \{(u,v,0,\epsilon) \; \forall u,v \in V_2\},$ where $\epsilon$ is the empty string denoting the correlations in the amount of stored key material, which is 0 \bing{what does the `0' represent here?}.   

On this stage, we build on $G_3$ based on the state of $G_2$. Specifically, if QKD succeeds between two linked nodes, which it does with probability $\frac{1}{4},$ then a bit is added to that that bank of key material, which is a correlated with full probability if the link was coherent \bing{rephrase?}. If the link was not coherent, then we assume that it became a fully mixed state, and that resulting measurements are random and therefore correlated with $\frac{1}{2}$ probability. Formally, this means that for each edge $(u,v,1) \in E_2$, with $\frac{1}{4}$ probability we update the corresponding edge $(u,v,k,c)$ in $E_3$ to $(u,v,k+1,c||0)$, and likewise for each edge $(u,v,0)$ we update the corresponding edge to $(u,v,k,c||0)$ or $(u,v,k,c||1)$  with equal probability, where $||$ denotes concatenation of bit strings.

\par
\textbf{4. Key Distillation}
Stages 1-3 repeat some $M$ times, building sufficiently sized key stores between each of the participating parties in our network until, on this stage, the final key-distillation and key-routing process occurs. On this stage, each pair of parties that share some amount of raw key material can conduct standard post-processing procedures, namely, error correction and privacy amplification, to transform their raw-key stores into secret-key stores. As we are limiting our analysis in this work to only consider the performance in the asymptotic key-length realm, we do not consider finite key effects, and so the simulator simply transforms the edges $(u,v,k,c)$ in $G_3$ to be $(u,v,(1-2h(Q))k, \epsilon)$, to signify the error correction and privacy amplification process according to the standard process, where Q is the quantum bit error rate of the key, calculated as $\frac{w(c)}{k}$, where $w(x)$ signifies the Hamming weight of the bit string $x$ and where $h(x)=x\log(x)-(1-x)\log(1-x)$ is the binary entropy function. 
Following this process, the network conducts the final routing process on $G_4$, obtained through the above transformations of edges, in an effort to route the maximum amount of key material from Alice to Bob. To do this, we use a standard max-flow algorithm, in which any flow of $n$ key-bits from node $a$ to node $b$ going through node $c$ signifies node $c$ publishing the XOR of $n$ bits from its key stores shared with $a$ and $b$ respectively, and then discarding those $n$ bits. Nodes $a$ and $b$ can then of course recover this key material, pushing it through the network until we culminate with the maximal amount of key material being shared by Alice and Bob. 


% \iffalse 
% \begin{figure}
%     \centering
%     \includegraphics{stage1.pdf}
%     \caption{The initial network, in a 5x5 grid, with a central trusted node (T) between Alice (A) and Bob (B), as discussed in stage 0.}
%     \label{fig:stage1}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics{stage2.pdf}
%     \caption{A possible network configuration after stage 1, in which some nodes succeed in establishing a shared EPR pair with their neighbors over the fiber channels and some do not. Note that there are a number of possible paths between A, B and T.  }
%     \label{fig:stage2}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics{stage3.pdf}
%     \caption{Successful entanglement chaining and routing (depicted as the intra-repeater connections) as discussed in stage 2. In this graph, routing has resulted in a channel being created between each pair of A, B and T. These routes are successful and coherent only if every bell state measurement along the path succeeds, and if no decohering occurs in the path, so minimizing the path lengths with effective routing algorithms and trusted node utilization is advantageous. For the purposes of this diagram we condition on the channels remaining coherent, but in practice any could have become decoherent. }
%     \label{fig:stage3}
% \end{figure}
% \fi 

\begin{figure}
    \centering
    \includegraphics{stage5.pdf}
    \caption{$G_3$ being modified, as discussed in stage 3, where $k_i$ denotes the number of key bits already shared between two nodes, and $c_i$ denotes the correlation bit string. This diagram assumes that QKD was successful on each of the error free channels established in Figure \ref{fig:stages1-3}(c).}
    \label{fig:stage5}
\end{figure}
% Stages 1-3 repeat some $M$ times, building sufficient key stores between each the participating parties in our network until, on this stage, the final routing and distillation of key material occurs. \OA{assuming we just go with simple trusted nodes here, and leave regular to journal if not in this one} On this stage, the network conducts a standard max-flow algorithm, with a slight variation, to determine how to route the maximum amount of key material from Alice to Bob through the weighted edges present in the graph. To "push" $n$ bits key material from Alice, through a trusted node, to Bob, the trusted node must first share at least $n$ bits of key material with both Alice and Bob. The trusted node then XORs the $n$ bit  key strings and publishes them, so that Alice and Bob can recover each others raw-key strings. Here it becomes clear why it is necessary that these intermediary nodes be trusted, as they, unlike the repeaters, are the only parties other than Alice and Bob that have full information on the key strings. Additionally, it is worthwhile to note that this XORing process can result in cascading errors when routing raw key material, and so we cannot simply chain trusted nodes infinitely using this method. For completeless, we look at how the secondary network graph evolves during this stage. Consider any two flows pushing $n$ bits from node $u$ through node $v$ to node $w$, the corresponding edges in $G_4$, which are originally equal to the edges of $G_3$, are updated from $(u,v,k_1, c_1),(v,w,k_2, c_2)$, and $(u,w,k_3, c_3)$ to
% $(u,v,k_1-n,c_1||_0^{k_1-n}),(v,w,k_2-n,c_2||_0^{k_2-n})$, and
% $(u,w,k_3+n, c_3 || (c_1 ||_{k_1-n}^{k_1} \oplus c_2 ||_{k_2-n}^{k_2})).$ 
% To allow this error information to cascade through the whole network we change the max-flow algorithm slightly so that, rather than executing each flow, we execute one flow, update the graph, and then re-run the algorithm. We repeat this until no more key-material can be pushed from Alice to Bob, and then we proceed with standard post-processing procedure: namely, error-correction and privacy amplification. 

% As in this work we only analyze the performance of this network in the asymptotic case, we do not concern ourselves with any finite key effects, and can instead calculate the overall key rate, as is standard,to be $1-2h(Q)$ where $h(x) = xlog(x) - (1-x)log(1-x)$ is the binary entropy function and $Q = \frac{w(c)}{K}$ where $w(x)$ is the hamming weight function and $c$ and $K$ are the bit string and weight associated with the edge connecting Alice and Bob in the finalized $G_4$ graph.


==> tex/one-trusted-node.tex <==
%wb, 5/10/2020, use a 2x2 plots to show the impacts of all the parameters
\begin{figure}[t]
	\centering
	%\vspace{-.1in}
	\subfigure[Impact of fiber length.]{%\label{subfig:pdf}]{%
		\includegraphics[width=0.24\textwidth]{figs/L_1TN.pdf}
	}
	\hspace{-.148in}
	\subfigure[Impact of decoherence rate.]{%
		\includegraphics[width=0.24\textwidth]{figs/E_1TN.pdf}
	} \\
	%\vspace{-.1in}
	\subfigure[Impact of BSM success rate.]{%
		\includegraphics[width=0.24\textwidth]{figs/Q_1TN.pdf}
	}
	\hspace{-.148in}
	\subfigure[Impact of network size.]{%
		\includegraphics[width=0.24\textwidth]{figs/S_1TN.pdf}
	}
	%\vspace{-.2in}
	\caption{Impact of various parameters on key rate when there is one trusted node in the network ($5 \times 5$ grid).}
	\label{fig:1TNGraphs}
\end{figure}

\subsection{Single Trusted Node} \label{sec:one-trusted-node}
We now consider the scenario where a single trusted node is placed at the center of the network grid, and investigate the impact of various parameters on key rate in this scenario. Figures~\ref{fig:1TNGraphs}(a)-(d) plot the key rate when varying the fiber length, decoherence rate, BSM success rate and network size, respectively. The results show that, under all three routing algorithms, having one trusted node leads to significantly higher key rate than the same setting with no trusted node (see Fig.~\ref{fig:NoTNGraphs}).
%Compared to the corresponding results with no trusted node (in Fig.~\ref{fig:NoTNGraphs}), we see  for the same setting. 
As an example, when there is no trusted node, as shown in Fig.~\ref{fig:NoTNGraphs}(a), the maximal key rate achieved for the global algorithm was .07 key-bits/round, while it is .3 key-bits/round, more than $3\times$ higher, as shown in Fig.~\ref{fig:1TNGraphs}(a) when there is one trusted node. 

Comparing Fig.~\ref{fig:1TNGraphs}(a) and Fig.~\ref{fig:NoTNGraphs}(a), we see that for the global algorithm,  when varying the fiber length from 1 to 15 km, the key rates with one trusted node are $.08$-$.25$
%$.25$-$.08$ 
higher than that with no trusted node under the same setting, corresponding to a $1.9$-$4.4\times$ increase; the corresponding increases in key rate for IA and NIA algorithms are $1.2$-$8.8\times$ and $2.1$ - $9.2\times$, respectively. 
%factor of $186\%$-$437\%$; the corresponding increases in key rate for IA and NIA algorithms are by factors of $116\%$-$886\%$ and $208\%$-$919\%$, respectively. \OA{Thoughts on this? The increase is huge as the No TN key rate drops lower, but the key rates themselves aren't that high.} 
In fact, with one trusted node and in the same setting, the NIA algorithm achieves greater key rates than even the global algorithm could with no trusted nodes. This is because the trusted node essentially reduces the ``size'' of the network, allowing shorter paths to be constructed between Alice/Bob and the trusted node, As the local algorithms have information on a higher fraction of the total network for smaller networks, this reduction in the effective size of the network has a particularly strong effect on the local algorithms. 
\iffalse 
With a baseline set, we now move to consider what one can do by adding a single trusted node to the network. Specifically, we repeat the host of simulations discussed previously, now with a trusted node located at the center of the network grid. What we find is that, while trends between parameters, algorithms, and key rate all remain constant, in every case the key rate is greatly increased by the addition the trusted node. Contrasting each of the sub-figures in Fig.~\ref{fig:1TNGraphs} with their respective counterparts in Fig.~\ref{fig:NoTNGraphs}, this increase in evident. Where, in Fig.~\ref{fig:NoTNGraphs}(a) the maximal key rate achieved for the global algorithm was .07 key-bits/round, in Fig.~\ref{fig:1TNGraphs}(a) it is more than threefold that at .3 key-bits/round. In fact, with one trusted node the NIA algorithm achieves greater key-rates than even the global algorithm could with no trusted nodes. 
\fi 
This trend is also exhibited in Figs.~\ref{fig:1TNGraphs}(b)-(d). Where, again comparing with their counterparts in Fig.~\ref{fig:NoTNGraphs}, we see that the addition of a trusted node results in an almost two-fold increase in maximum achievable key-rate for the cases of decoherence, BSM success rate and network size. 

\iffalse Interestingly, we see that the difference in performance between the global and IA algorithms becomes less pronounced in these cases, while it was not the case in the results when varying the fiber length as shown in Fig.~\ref{fig:1TNGraphs}(a). This is likely due to the fact that, when varying fiber length, the global algorithm is able to find longer paths that the local algorithms cannot find as the length (and therefore edge-sparsity) increases. On the other hand, when varying decoherence, BSM rate or network size, the optimal paths remain easy to find. And, as they are in general shorter (and therefore easier to find) when they are between Alice/Bob and a trusted node than when they are simply between Alice and Bob (i.e., when there is no trusted node), the difference between the global and IA algorithm is, understandably, less. \OA{This doesn't actually look to be true, or i'm confused by what I meant}
\fi
% With the addition of a single central trusted node, the capabilities of our protocol are greatly increased. To demonstrate this, we run another host of simulations, comparable to the ones in the previous section, but with a trusted node located in the center of the grid, as shown in Figures \ref{fig:1TNGraphs} and \ref{fig:1TNGraphs2}. Across each scenario we find that the addition of a single trusted node can more than double the key rate of the overall protocol. Most strikingly, when comparing Figures \ref{fig:NoTNGraphs}(a) and \ref{fig:1TNGraphs}(a), we see an order of magnitude increase in the achievable key rate.  Further, there remains a significant advantage to be had by using the IA algorithm over the NIA algorithm, and in fact, with a central trusted node, the IA algorithm is closer in performance to the global algorithm than it was when there were no trusted nodes. 

In Fig.~\ref{fig:NoiseLevels}, we show the performance of the three algorithms with no trusted nodes and one trusted node in two additional channel scenarios: perfect BSM success probability with 2\% decoherence and 85\% BSM success probability with 5\% decoherence. In  Fig.~\ref{fig:NoiseLevels}(a), we see that even with the elimination of BSM failures, as the length increases between nodes the key rate still drops significantly. We see that even the NIA algorithm with a central trusted node (TN) outperforms the global algorithm with no TN, as the shorter paths between the parties and the TN are simply more likely to exist than the longer paths that must exist to connect Alice and Bob in the no TN case. In  Fig.~\ref{fig:NoiseLevels}(b) we consider a less idealized scenario, in which the BSM probability is our default of $85\%$ and our decoherence rate is higher, at $5\%$. We see that for this scenario, not even the global algorithm can achieve a positive key rate for the no TN case (at least in $10^6$ rounds of the network), and that in general the key rates achieved by the central TN is significantly lower (between $5-10\times$) than was achieved with $2\%$ decoherence in Fig.~\ref{fig:1TNGraphs}(a). It is notable, however, that in Fig.~\ref{fig:NoiseLevels}(b) we see that using 1 TN, each algorithm is able to maintain a positive key rate even when there is a 5\% decoherence rate, and Alice and Bob  are separated by 113 km (when $L=20$ km, considering a $5\times5$ network grid).


%% We note that with 5\% decoherence, not even the global algorithm can achieve a positive key rate for the no trusted node configuration
\tydubfigsingle{figs/L_01_5x5.pdf}{100\% BSM Success Prob.}{figs/E5_1TN.pdf}{5\% decoherence rate}{(a) The capabilities of the network when operating in an idealized scenario with no BSM failures (i.e. perfect repeaters) and 2\% decoherence probability. (b) The capabilities of the network with 5\% decoherence probability and 85\% BSM success probability.}{NoiseLevels}




==> tex/perf.tex <==
\section{Performance Evaluation} \label{sec:perf}
%We are now in a position to evaluate the performance of the proposed QKD network using our various routing algorithms. We will compare the performance of each algorithm in number of different scenarios and configurations, and attempt to draw lessons about

In this section, we evaluate the performance of quantum key distribution in quantum networks using the various routing algorithms. We will compare the performance of the algorithms in a number of settings and investigate the impact of various parameters on the performance.

\subsection{Evaluation Setup}
We consider the scenarios where Alice and Bob are placed at the two corners of an $N\times N$ grid.  
The parameters related to network topology include the size of the grid ($N$) and the length of the fiber channel of each edge (horizontal or vertical) of the grid ($L$). The quality of the quantum network is represented by the probability of a successful Bell state measurement (BSM) at a repeater ($B$), and the probability of decoherence ($D$, see Equation \ref{eq:shared-state}).   Note that $L$ is the fiber length between neighboring two nodes.  Since Alice and Bob are at opposite corners of the entire grid network, the actual distance, therefore, between the two users is actually $\sqrt{2}(N-1) L$.
Table~\ref{tab:defaults} summarizes these parameters, with their default values and range of the values.  
%We provide a table with default values in Table~\ref{fig:defaults}.
%We further investigate the impact of various parameters related to network topology and quality of the quantum network, including the size of the grid ($N$), the length of the fiber channel of each edge (horizontal or vertical) of the grid ($L$), the probability of a successful Bell state measurement at a repeater ($B$), and the probability of an EPR pair becoming decoherent ($D$). 


%The probability a photon is successfully transmitted along $L$ km of fiber is $10^{-.15L/10}$. 

\begin{table}
    \centering
%    \begin{center}
    %\caption{A table providing the default values for each of the network parameters and a description of the parameters.}
%    \caption{Parameters and settings of the parameters used in performance evaluation. }
    \caption{Parameters explored in performance evaluation. }
        \begin{tabular}{| c | c | c | p{3.8cm}|} 
        \hline
        \textbf{Parameter} &  \textbf{Default} & \textbf{Range} & \textbf{Description} \\ \hline
        $N$ & 5    & 5 - 15       & The network consists of $N^2$ nodes arranged in an $N \times N$ grid. \\ \hline
        $L$ & 1 km & 1 - 20 km & The length of the fiber connecting neighboring nodes. The distance between Alice and Bob scales with both $N$ and $L$.  \\ \hline
        $B$ & .85  & 0.65 - 1.00  & Represents the quality of the repeaters. A Bell state measurement succeeds at a repeater with probability $B$. \\ \hline
        $D$ & .02  & 0.00 - 0.06  & Represents the amount of noise in the channels. EPR pairs decohere with probability $D$. \\
        \hline
        \end{tabular}
%    \end{center}
    \label{tab:defaults}
\end{table}
%The default values for these parameters are $N = 5$, $L = 1$ km, $B = .85$, and $D = .02$. \WK{Put these in a table with text descriptions of what they mean for easier reference throughout this section.} We investigate the impact of one parameter by varying that parameter, while setting the other parameters as the default values. 


The performance metric is {\em key rate}, i.e., the average number of secret key-bits generated between Alice and Bob per round of network use as discussed in Section \ref{sec:model}. Unless otherwise stated, the number of rounds we simulate for each test and for each setting is $10^6$. We also evaluate the network's performance when there are no trusted nodes; a single trusted node; and two trusted nodes, along with different location configurations.
%to investigate the impact of the number of trusted nodes on key rate. 
%%In the following, we first present the results when there are no trusted nodes. We then present the results when there is a single trusted node, placed in the center of the grid. Last, we present the results when there are two trusted nodes, and investigate the impact of their placement in the grid on the resulting key rate.  

\subsection{No Trusted Nodes}
%\triplefigbig{L_noTN.png}{Variable: Fiber Length (km)}{E_noTN.png}{Variable: Decoherence Rate}{Q_noTN.png}{Variable: BSM Rate}{These charts plot the ratio of secret key-bits obtained per iteration over 100,000 iterations, with one free parameter in each chart. The default values are a fiber length of 1 (and thus a probability of successful transmission of $10^{-.15/10}$), an error rate of .02, and a BSM success probability of .85, with a 5x5 network grid where Alice and Bob are located at opposite corners with no trusted nodes.}{NoTNGraphs}

%wb, 5/10/2020, use a 2x2 plots to show the impacts of all the parameters
\begin{figure}[t]
	\centering
	%\vspace{-.1in}
	\subfigure[Impact of fiber length.]{%\label{subfig:pdf}]{%
		\includegraphics[width=0.24\textwidth]{figs/L_noTN.pdf}
	}
	\hspace{-.148in}
	\subfigure[Impact of decoherence rate.]{%
		\includegraphics[width=0.24\textwidth]{figs/E_noTN.pdf}
	} \\
	%\vspace{-.1in}
	\subfigure[Impact of BSM success rate.]{%
		\includegraphics[width=0.24\textwidth]{figs/Q_noTN.pdf}
	}
	\hspace{-.148in}
	\subfigure[Impact of network size.]{%
		\includegraphics[width=0.24\textwidth]{figs/S_noTN.pdf}
	}
	%\vspace{-.2in}
	\caption{Impact of various parameters on key rate when there is no trusted node in the network ($5 \times 5$ grid). Note, as discussed, ``fiber length'' $L$ is the length between nodes.  Thus, the actual distance between the two users is actually $\sqrt{2}(N-1) L$.}
	\label{fig:NoTNGraphs}
\end{figure}


\iffalse 
\begin{figure}[t]
	\centering
	%\vspace{-.1in}
	\subfigure[Key rate vs. fiber length.]{%\label{subfig:pdf}]{%
		\includegraphics[width=0.24\textwidth]{figs/L_noTN.pdf}
	}
	\hspace{-.148in}
	\subfigure[Key rate vs. decoherence rate.]{%
		\includegraphics[width=0.24\textwidth]{figs/E_noTN.pdf}
	} \\
	%\vspace{-.1in}
	\subfigure[Key rate vs. BSM success rate.]{%
		\includegraphics[width=0.24\textwidth]{figs/Q_noTN.pdf}
	}
	\hspace{-.148in}
	\subfigure[Key rate vs. network size.]{%
		\includegraphics[width=0.24\textwidth]{figs/S_noTN.pdf}
	}
	%\vspace{-.2in}
	\caption{Impact of various parameters on key rate when there is no trusted node in the network ($5 \times 5$ grid).}
	\label{fig:NoTNGraphs}
\end{figure}
\fi 

%\triplefigbig{figs/L_noTN.png}{Key rate vs. fiber length (km).}{figs/E_noTN.png}{Key rate vs. decoherence rate.}{figs/Q_noTN.png}{Key rate vs. BSM rate.}{Impact of various parameters on key rate when there is no trusted node in the network ($5 \times 5$ grid). }{NoTNGraphs}

%\tydubfigsingle{figs/S_noTN.png}{Variable: Size}{figs/L_noTNE0.png}{Variable: Length with 0\% Decoherence}{These charts provide some additional insight into the performance of our model with the default parameters mentioned in Figure \ref{fig:NoTNGraphs}, with no trusted nodes. a) Demonstrates the drop in performance, shared by all algorithms, as the network size increases and therefore the overall error and probability of a path failing increases while b) shows the capabilities of the network when operating in an idealized scenario with no decoherence probability }{NoTNGraphs2}


We first investigate the scenario with no trusted node and only repeaters. These results serve as baselines to demonstrate the benefits of having trusted nodes in the network in Sections~\ref{sec:one-trusted-node} and \ref{sec:more-trusted-nodes}. Fig.~\ref{fig:NoTNGraphs}(a) plots the key rate when varying the fiber length, $L$, for a $5 \times 5$ grid. The results of the three routing algorithms are plotted in the figure. As expected, since increasing the fiber length leads to higher fiber loss, the key rate decreases with $L$. The global routing algorithm, also as expected, outperforms the two local algorithms. Between the two local algorithms, the intersection-avoidance (IA) algorithm significantly outperforms non-intersection-avoidance (NIA) algorithm, particularly for lower fiber lengths.
% The difference between these two localized algorithms is particularly significant for lower values of fiber length. 
The difference between the global algorithm and IA algorithm is small for short fiber length, and increases when the fiber length increases, where having global knowledge allows the algorithm to find paths, even when they are longer and more complicated.
%enables the network to ensure that it is finding paths, even when they are longer and more complicated. 

Fig.~\ref{fig:NoTNGraphs}(b) plots key rate when increasing the decoherence rate $D$. We again observe that the global routing algorithm outperforms the two local algorithms, and the IA algorithm significantly outperforms the NIA algorithm.
%and between the two local algorithms, the IA algorithm significantly outperforms the NIA algorithm.
%find that the expected hierarchy between algorithms holds, with the global outperforming the local algorithms, and the IA algorithm out performing the IA algorithm. 
%Similarly, as we would expect, the key rate drops, rather drastically, as the decoherence rate increases. 
As expected, increasing the decoherence rate leads to lower key rates; the decrease is particularly dramatic when increasing the decoherence rate from 0 to 2\%. As an example, for the global routing algorithm, the key rate decreases from .3 key-bits/round to just over .07 key-bits/round when increasing the decoherence rate from 0 to 2\%.
%In fact, when increasing the decoherence rate from 0\% to 2\%, as it was in  Fig.~\ref{fig:NoTNGraphs}(a), we see, for the global algorithm, a drop from a key rate of .3 key-bits/iteration to just over .07 key-bits/iteration.
We also note that, interestingly, while both the global and IA algorithms achieve a key rate around .07 at 2\% decoherence, the NIA algorithms, under the ideal condition of 0\% decoherence, achieves the same key rate of .07 key-bits/round. 
The drastic advantage of the IA algorithm over the NIA algorithm highlights the importance of designing effective local routing algorithms.
%Once again we see that the IA algorithm has a drastic advantage over the NIA algorithm, highlighting the importance of designing effective routing algorithms.

%We conduct a similar investigation in  Fig.~\ref{fig:NoTNGraphs}(c), this time varying the probability that the bell state measurement at each repeater succeeds. 
Fig.~\ref{fig:NoTNGraphs}(c) plots key rate when varying $B$, the probability that the Bell state measurement at a repeater succeeds. The relative performance across the three routing algorithms is similar as the above two scenarios. 
%We again observe similar relative performance across the three routing algorithms. 
%, the expected patterns hold. 
Of note, it is evident 
%from this analysis 
that increasing the reliability of these measurements can lead to a significantly improved key rate. At a 75\% success rate, for example, the global algorithm achieves just under .026 key-bits/second, but an increase to 95\% or even 100\% success rates allows us to achieve key rates of approximately .153 and .216 respectively. 

Last, Fig.~\ref{fig:NoTNGraphs}(d) demonstrates the impact of network size $N$ on key rate.  Note that, by increasing $N$ (the number of nodes in the network) but keeping the horizontal/vertical distance between two adjacent nodes fixed at 1 km, we are effectively increasing the total distance between Alice and Bob (they are at the two corners of the grid). For all the routing algorithms, the key rate decreases when the network size (i.e., total distance) increases. This is expected since, as the network size increases, the path between Alice and Bob becomes longer,
%(they are at the two corner of the grid), 
and therefore the overall error (see Equation \ref{eq:shared-state}) and probability of a path failing increases, leading to lower key rate. Of the three routing algorithms, the global algorithm is less affected compared with the other two algorithms since it is more capable of finding longer paths as the network size increases than the two local algorithms.

We observe that, as the distance between the end users $A$ and $B$ increases, even using quantum repeaters with perfect internal performance (i.e., $B = 1$), the efficiency of the entire network degrades rapidly (we shall discuss this further in in Fig.~\ref{fig:NoiseLevels}).  We show in the following sections how even a single trusted node can dramatically improve the performance of QKD, indicating that, even in the future as repeater technology becomes more prevalent, trusted nodes may still be necessary to ensure high key rate when the distance between end users is significant.


%Note that this effectively shows that, as distance between the end users $A$ and $B$ increases, even using quantum repeaters with perfect internal performance (i.e., $B = 1$ as we'll see in Fig.~\ref{fig:NoiseLevels}), the efficiency of the entire network degrades rapidly.  We show in the following sections how even a single trusted node can dramatically improve performance showing that, even in the future as repeater technology becomes more prevalent, trusted nodes may still be necessary to ensure high speed communication.



%Additionally, in Fig.~\ref{fig:NoTNGraphs2}(a), we investigate the last network parameter: network size. We find that as the number of nodes increases, the key rate decreases. This trend holds for each of the algorithms, but the global algorithm, as it is more capable at finding longer paths than the local algorithms, is not hindered by size as much as the local algorithms. Finally, we consider an idealized case, shown in Fig.~\ref{fig:NoTNGraphs2}(b), in which the probability of decoherence in the channel is 0\%.

% This chart hint, taken alongside the charts we have looked at thus far, hint at a larger limitation we saw in the data. As the fiber l
% As one might expect, for each algorithm, the obvious relation between each parameter and the key rate hold: there is an inverse correlation of the key rate with of $L,E,$ and $n$, and a direct correlation with $B$. We show this data, for each of our algorithms, in figures \ref{fig:NoTNGraphs} and \ref{fig:NoTNGraphs2}(a). In addition, we consider the effect of keeping the overall physical covered by the network constant, such that having additional nodes lowers the physical distance traveled in each hop, as shown in Figure \ref{fig:0TNFixed}. What we find by doing this is that, in fact, the advantage provided by this is limited due to the compounding nature of the error across each hop --- indeed, we find that more than any other factor, error is the limiting parameter in all of our tests, followed by the size of the network. With this in mind, we have also conducted an analysis of the performance of our algorithms in an error free network environment, as shown in Figure \ref{fig:NoTNGraphs}(b). 

% We note here the clear advantage that our Intersection Avoidant (IA) algorithm has over the Non-Intersection avoidant variant (NIA). The global algorithm, as expected, out performs both, especially as fiber length increases (and thus, the optimal paths between parties likely become more complex increases), but in many scenarios the IA algorithm out performs the NIA algorithm by a greater margin than that of the global to the IA algorithm. 




\input{one-trusted-node}

\input{more-trusted-node}


